State-Novelty Guided Action Persistence in Deep Reinforcement Learning

While a powerful and promising approach, deep reinforcement learning (DRL) still suffers from sample inefficiency, which can be notably improved by resorting to more sophisticated techniques to address the exploration-exploitation dilemma. One such technique relies on action persistence (i.e., repeating an action over multiple steps). However, previous work exploiting action persistence either applies a fixed strategy or learns additional value functions (or policy) for selecting the repetition number. In this paper, we propose a novel method to dynamically adjust the action persistence based on the current exploration status of the state space. In such a way, our method does not require training of additional value functions or policy. Moreover, the use of a smooth scheduling of the repeat probability allows a more effective balance between exploration and exploitation. Furthermore, our method can be seamlessly integrated into various basic exploration strategies to incorporate temporal persistence. Finally, extensive experiments on different DMControl tasks demonstrate that our state-novelty guided action persistence method significantly improves the sample efficiency.

==> point-by-point-response.tex <==
\noindent 
\begin{answereditor}{
Decision: Minor revision.
We invite you to revise your paper. When your revision is ready, please submit the updated manuscript and a point-by-point response.}

\noindent Dear Editor, Dear Reviewers,

Thank you for considering the value of our work and providing your valuable feedback.
Your thoughtful comments help us improve the original manuscript.
With your feedback, we made revisions in the paper and included more experiments to strength the contributions of our paper. 
%
More precisely, we conducted the following revisions according to the feedback:
\begin{itemize}
    \item We trained the agents until convergence for comparing the convergence rewards. \textbf{(Reviewer 1)}
    \item  We compared different schedulers to decide the probability of action persistence. 
    We tested the linear scheduler and sigmoid scheduler. \textbf{(Reviewer 1)}
    \item We compared different measures for state novelty.
    We tested quantized states and k-means clustering. \textbf{(Reviewer 1)}
    \item We further added point-to-point detailed explanations for the remaining questions. \textbf{(Reviewer 1 and Reviewer 2) }
\end{itemize}
% Additionally, we thank the interesting question from Reviewer 2 and provide our answer to it.

Finally, we are grateful for all of the feedback from the reviewers and the Editor, and appreciate the efforts and the suggestions for improvements.
Below we provide detailed responses to the reviewer comments. 
\end{answereditor}
\vspace{2ex}
\noindent\textbf{Reviewer 1}\\

\noindent\textbf{Comments:}
This paper tackles the exploration-exploitation dilemma by exploring the impact of action persistence.
To this end, the paper proposes an algorithm that dynamically adjusts the probability of repeating the last action to optimize learning.
Experimental results demonstrate faster convergence compared to baseline methods.
However, further improvements are needed in the ablation studies to provide stronger justification for the proposed method.
I believe revision could significantly enhance the clarity and soundness of this work. \\

\noindent\textbf{Answer:} Thank you so much for highlighting the strength of our paper and providing your valuable feedback.
We totally agree that following the suggestions from you could enhance our work.
We have included more experiments in the paper according to your feedback, as detailed below.

\bigbreak

\noindent\textbf{R1-Q1:}
While the results depicted in Figure 4 show promise, it appears that the rewards have not yet converged. The convergence reward is also important, although the proposed method can reach a higher reward in the early stages. \\

\noindent\textbf{Answer:}
We agree it makes sense to also compare the convergence rewards.
We further train the three agents in \Cref{fig:different repeat} longer, as shown in \Cref{fig:convergence} in \refcm{R1Q1-2}.
According to the results, our method still outperforms using fixed action persistences with respect to the convergence rewards.

\bigbreak

\noindent\textbf{R1-Q2:}
Although the concept of adjusting the probability of action persistence is intuitive, comparing it with baselines that control this probability could further validate the effectiveness of the proposed methods. For example, gradually decreasing the probability based on the number of episodes using a linear or sigmoid scheduler could provide insights. Given the findings from Figure 4, it would be interesting to see if a simpler logarithmic or sigmoid scheduler could achieve similar performance. \\

\noindent\textbf{Answer:}
To answer this question, we have run some additional experiments using a linear scheduler and a sigmoid scheduler to decide the probability of repeating the actions.
Both the evaluation curves and corresponding probabilities along the training are shown in \Cref{fig:scheduler} in \refcm{R1Q2Q3-2}.
Our method outperforms the baselines of using a simple scheduler for deciding the probability.
Notably, our method has a smaller variance in the results.
It is possible that tuning the hyperparameters and the type of scheduler could achieve a similar performance compared to our method.
However, our method is intuitive and does not require task-dependent hyperparameter-tuning.

\bigbreak

\noindent\textbf{R1-Q3:}
The author proposes a persistence adaptor and applies an image encoder and binary state coding to compute the state novelty. To strengthen the justification for these choices, it would be beneficial for the authors to compare this approach with simpler baselines, such as quantized states or k-means clusters. This comparison would provide additional insights into the design of the encoder and the method of computing state novelty.
\\

\noindent\textbf{Answer:}
To show the robustness of our method with respect to
the design choice of measuring the state novelty, we run experiments of using quantized states and k-means clustered states for pseudo count, as shown in \Cref{fig:different_count} in \refcm{R1Q2Q3-2}.
Our method is stable even when changing the state novelty measure.

\clearpage
\noindent\textbf{Reviewer 2}\\

\noindent\textbf{Comments:}
This paper addresses the issue of sample inefficiency in deep reinforcement learning (DRL) by proposing a novel method to dynamically adjust action persistence based on the exploration status of the state space. Traditional methods either use fixed strategies or require additional value functions for action persistence, leading to increased computational complexity. The proposed method, called State-Novelty guided Action Persistence (SNAP), evaluates the novelty of each state and adjusts action repetition accordingly, thereby enhancing exploration without the need for extra value functions or policies. This approach integrates smoothly with various exploration strategies and has demonstrated significant improvements in sample efficiency through extensive experiments on DMControl tasks.

\noindent Overall, I think the main idea is persuasive and well motivated. Please address the comments in the other review to further strengthen the contribution of the paper. \\

\noindent\textbf{Answer:}
Thank you very much for reviewing our paper given the limited time and recognizing the main idea of our paper.
We have addressed the comments from Reviewer 1.
Please check our answers to Reviewer 1 above.
We also provide our detailed answer to your interesting question below.

\bigbreak

\noindent\textbf{R2-Q1:}
There remains a question of my own: I think state-novelty alone is not sufficient to determine action persistence. Actually, it should be determined whether the policy has been sufficiently converged on the state - e.g. for some state, it may be very difficult to learn the optimal action (many updates required) because there is a very similar state with a very different optimal action. Could we use bellman error or something similar as a surrogate measure of policy / value convergence? if not, why?\\

\noindent\textbf{Answer:}
We thank the reviewer for this thought-provoking question.

\textbf{Why state-novelty: }
We design action persistence to help the agent to quickly reach far-away novel states by repeatedly moving in some direction, thereby enhancing exploration (as shown in \Cref{fig:pure exploration and coverage of state space}), not specifically to learn the optimal action for some ”hard” states quickly.
For this goal, state novelty is a natural measure to guide the action persistence for discovering more states or increasing the state coverage within a certain number of steps.

\textbf{Why not policy/value convergence: }
Using a measure of policy/value convergence to decide the number of repetition is definitely an interesting idea.
However, we believe that in general, action persistence may hinder policy/value convergence, since an optimal policy may take different actions in consecutive states.
This is why the probability of action persistence decreases to zero in the proposed method.
% Instead, convergence is more related to replay ratio
% Increasing the replay ratio (i.e., the number of updates per iteration) \citep{d'oro2023sampleefficient} is proven to be significant for improving sample-efficiency.
% However, the primacy bias \citep{nikishin2022primacybiasdeepreinforcement} or plasticity loss is known to be the bottleneck of further improving the sample efficiency, as the the replay ratio continues to increase.
% The Bellman error might be used to decide how many updates we should make on each state such that it could help mitigate the primacy bias or plasticity loss for higher sample efficiency.

\clearpage

